ARM: Any-Time Super-Resolution Method

This paper proposes an Any-time super-Resolution Method (ARM) to tackle the over-parameterized single image super-resolution (SISR) models. Our ARM is motivated by three observations: (1) The performance of different image patches varies with SISR networks of different sizes. (2) There is a tradeoff between computation overhead and performance of the reconstructed image. (3) Given an input image, its edge information can be an effective option to estimate its PSNR. Subsequently, we train an ARM supernet containing SISR subnets of different sizes to deal with image patches of various complexity. To that effect, we construct an Edge-to-PSNR lookup table that maps the edge score of an image patch to the PSNR performance for each subnet, together with a set of computation costs for the subnets. In the inference, the image patches are individually distributed to different subnets for a better computation-performance tradeoff. Moreover, each SISR subnet shares weights of the ARM supernet, thus no extra parameters are introduced. The setting of multiple subnets can well adapt the computational cost of SISR model to the dynamically available hardware resources, allowing the SISR task to be in service at any time. Extensive experiments on resolution datasets of different sizes with popular SISR networks as backbones verify the effectiveness and the versatility of our ARM. The source code is available at https://github.com/chenbong/ARM-Net.

==> img/tab_Ablation.tex <==
\begin{table}[t]
\caption{The results of ablation experiments.}
\label{tab:ablation}
\centering
\resizebox{.9\linewidth}{!}
{
\begin{tabular}{c|c|c|c} 
\toprule
\multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Ablation\\\end{tabular}} & PSNR & FLOPs \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Subnet\\Num.\end{tabular}} & 2 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & 3 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & 5 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & 8 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Subnet\\Ratio\end{tabular}} & 1:1:1 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & 1:2:3 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & 1:4:9 & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Priori\\Distribution\end{tabular}} & Bin Avg. & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & Bin Mode & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\ 
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Edge\\Operator\\(Corr.)\end{tabular}} & Sobel(0.xx) & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & Canny (0.xx) & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & Roberts (0.xx) & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
 & Laplacian (0.85) & xx.xx / xx.xx / xx.xx & xxxx / xxxx / xxxx \\
\bottomrule
\end{tabular}
}
\end{table}
